Causality-Inspired Taxonomy for Explainable Artificial Intelligence

As two sides of the same coin, causality and explainable artificial intelligence (xAI) were initially proposed and developed with different goals. However, the latter can only be complete when seen through the lens of the causality framework. As such, we propose a novel causality-inspired framework for xAI that creates an environment for the development of xAI approaches. To show its applicability, biometrics was used as case study. For this, we have analysed 81 research papers on a myriad of biometric modalities and different tasks. We have categorised each of these methods according to our novel xAI Ladder and discussed the future directions of the field.

==> table_methods3.tex <==
% THE IDEA OF THIS TABLE IS TO SHOW SOME METHODS THAT SAY THAT ARE USING EXPLAINABILITY AND UNDERSTAND HOW THEY”SEE”EXPLAINABILITY. TO SHOW THE DIVERGENCE OF IDEAS AND THE LACK OF STANDARDS
% \begin{landscape}
% \begin{longtable}[h!]
%     \centering
%     \caption{Methods that leverage explainability methods to inspect the predictions of biometric systems. Some of these methods, promote interpretability through the usage of certain techniques, whereas others focus mostly on explaining the predictions. }
%     \label{tab:xai4bio_works}
%     \begin{tabular}{lclll}
%     \toprule
%         \textbf{Method} & \textbf{Year} & \textbf{Modality} & \textbf{Promote Interpretability} & \textbf{xAI Method} \\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Face Recognition}}} \\
%     \midrule
%     Yin~\textit{et al.}~\cite{yin2019towards} & 2019 & Face Recognition &  Feature and Spatial Activation Diversity loss & Locations of Filter Response \\
%     Zee~\textit{et al.}~\cite{zee2019enhancing} & 2019 & Face Recognition & Siamese training & Guided Backpropagation \& CAM \\
%     Williford~\textit{et al.}~\cite{williford2020explainable} & 2020 & Face Recognition & DISE, subtree EBP & Inpainting game \\
%     Neto~\textit{et al.}~\cite{neto2021my,neto2021focusface} & 2021 & Masked Face Recognition & Strong Constraints & Grad-CAM\\
%     Jiang and Zeng~\cite{jiang2021explainable} & 2021 & Face Recognition &  Local Feature Refine and Self-Attention based Reconstruction modules & Similarity Matrix \\
%     Liu~\textit{et al.}~\cite{liu2021heterogeneous} & 2021 & Heterogeneous Face Recognition & Symmetric adversarial loss & HFIDR \\
%     \textcolor{orange}{Anghelone~\textit{et al.}~\cite{anghelone2021explainable}} & 2021 & Face Recognition &  & \\
%     Mery~\textit{et al.}~\cite{mery2022black} & 2022 & Face Verification & - & Saliency maps AVG contours \\
%     \textcolor{red}{Fu~\textit{et al.}~\cite{fu2022explainability}} & 2022 & \textcolor{red}{Face quality for Face recogniton} & & \\
%     Han~\textit{et al.}~\cite{han2022personalized} & 2022 & Face Recognition & Personalized Kernels & Feature Maps \\
    

%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Face PAD}}} \\
%     \midrule
%     Liu~\textit{et al.}~\cite{liu2018learning} & 2018 & Face PAD & Aux. Supervision & - \\
%     Jourabloo~\textit{et al.}~\cite{jourabloo2018face} & 2018 & Face PAD & Spoof Pattern Estimation & t-SNE \\
%     Yang~\textit{et al.}~\cite{yang2019face} & 2019 & Face PAD & Aux. Supervision & t-SNE \\
%     Pinto~\textit{et al.}~\cite{pinto2020leveraging} & 2020 & Face PAD & - & Grad-CAM \\
%     Liu~\textit{et al.}~\cite{liu2020disentangling} & 2020 & Face PAD & Aux. Supervision & - \\
%     Shao~\textit{et al.}~\cite{shao2020regularized} & 2020 & Face PAD & Depth-Map Estimation & Attention Maps Visualisation \\
%     Wang~\textit{et al.}~\cite{wang2020deep} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE~\cite{JMLR:v9:vandermaaten08a} \\
%     Yu~\textit{et al.}~\cite{yu2020searching} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE \\
%     Sequeira~\textit{et al.}~\cite{sequeira2021exploratory} & 2021 & Face PAD & - & Grad-CAM \\
%     Aghdaie~\textit{et al.}~\cite{aghdaie2021attention} & 2021 & Face PAD & Attention & Attention Maps Visualisation \\
%     Chen~\textit{et al.}~\cite{chen2021dual} & 2021 & 3D Mask Face PAD & - & Grad-CAM and t-SNE \\
%     Neto~\textit{et al.}~\cite{neto2021myope} & 2021 & Face PAD & - & Grad-CAM \\
%     \textcolor{orange}{Fang~\textit{et al.}~\cite{fang2022learnable}} & 2022 & Face PAD & Attention & t-SNE \\
%     \textcolor{red}{Wang~\textit{et al.}~\cite{wang2022disentangled}} & 2022 & Face PAD & Spoof Maps & t-SNE\\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Iris PAD}}} \\
%     \midrule
%     Trokielewicz~\textit{et al.}~\cite{trokielewicz2018presentation} & 2018 & Cadaver Iris PAD & - & Grad-CAM and Guided backpropagation  \\
%     Sharma~\textit{et al.}~\cite{sharma2020d} & 2020 & Iris PAD & - & t-SNE and Grad-CAM \\
%     Fang~\textit{et al.}~\cite{fang2021iris} & 2021 & Iris PAD & Aux. Supervision, Attention &  Score-Weighted CAM~\cite{zhang2021group}\\
%     Chen~\textit{et al.}~\cite{chen2021} & 2021 & Iris PAD & Attention & Grad-CAM \\
%     \textcolor{purple}{Sharma and Ros}s~\cite{sharma2021viability} & 2021 & Iris PAD& - & Grad-CAM and t-SNE \\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Others}}} \\
%     \midrule
%     \textcolor{purple}{Genovese}~\textit{et al.}~\cite{Genovese2019} & 2019 & Face Aging & - & CGFSI \\
%     Trokielewicz~\textit{et al.}~\cite{trokielewicz2019perception} & 2018 & Cadaver Iris Recognition& -  & Grad-CAM \\
%     Hu~\textit{et al.}~\cite{hu2020end} & 2020 & Iris Recognition & - & Grad-CAM \\
%     Kao~\textit{et al.}~\cite{Kao2020AnOS} & 2020 & Signature Verification & - & - \\
%     Pinto~\textit{et al.}~\cite{pinto2020xecg} & 2020 & ECG Biometric Identification & - & Miscellaneous\\
%     Ahmed~\textit{et al.}~\cite{ahmed2020race} & 2020 & Race Estimation & - & Grad-CAM \\
%     Chowdhury~\textit{et al.}~\cite{chowdhury2020can} & 2020 & Fingerprint Recognition & - & Grad-CAM \\
%     Chandaliya and Nain~\cite{chandaliya2021child} & 2021 & Face Age Estimation & Attention & - \\
%     Joshi~\textit{et al.}~\cite{Joshi2021} & 2021 & Fingerprint ROI Segmentation & Monte Carlo Dropout & Uncertainty Map \\
%     \textcolor{purple}{Seibold}~\textit{et al.}~\cite{seibold2021focused}& 2021 & Face Morphing Attack Detection & Focused LRP & Focused LRP \\
%     Ortega~\textit{et al.}~\cite{ortega2021symbolic} & 2021 & Automatic Recruitment & LFIT~\cite{Ribeiro2016StudiesOL} & Declarative Explanation \\
%     Algermissen and H{\"o}rnlein~\cite{algermissen2021person} & 2021 & Footstep Person Recognition & - & Grad-CAM \\
%     Alshazly~\textit{et al.}~\cite{alshazly2021towards} & 2021 & Ear Recognition & - & Guided Grad-CAM \\
%     \textcolor{orange}{Mazaheri~\textit{et al.}~\cite{mazaheri2022detection}} & 2022 & Face Manipulation Detection & - & Grad-CAM \\
%     \textcolor{purple}{Kuehlkamp~\textit{et al.}~\cite{kuehlkamp2022interpretable}} & 2022 & Cadaver Iris Recognition & - & Segmentation Masks and CAM \\
%     \textcolor{orange}{Gelberg~\textit{et al.}~\cite{gelberg2022skeleton}} & 2022 & Typing style Recognition & Joint-based recognition & t-SNE \\
%     \textcolor{purple}{Xu~\textit{et al.}~\cite{xu2022supervised}} & 2022 & DeepFake Detection & -  & UMAP and Heatmaps \\
         

         
         
         


%     \bottomrule
%     \end{tabular}
    
% \end{longtable}
% \end{landscape}

\begin{landscape}
\begin{center}\begin{small}
\begin{longtable}{|p{0.22\textheight}p{0.02\textheight}p{0.25\textheight}p{0.25\textheight}p{0.35\textheight}|}

    \caption{Methods that leverage explainability methods to inspect the predictions of biometric systems. Some of these methods, promote interpretability through the usage of certain techniques, whereas others focus mostly on explaining the predictions.}\label{tab:xai4bio_works}\\
    \toprule
    \textbf{Method} & \textbf{Year} & \textbf{Modality} & \textbf{xAI Ladder} & \textbf{Approach to xAI} \\
    \hline
    \endhead

    %\endfoot
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Face Recognition}}} \\
    \hline
    \textcolor{blue}{Huber~\textit{et al.}~\cite{huber2024efficient}} & 2024 & Face Verification & Rung 2 - I. I. + I. P. & Decision-based Patch Replacement and Individual Dimension Contribution to Decision\\
    \textcolor{blue}{Li~\cite{li2023bionet}} & 2023 & Face Recognition & Rung 2 - M. P. & Biologically Inspired Architecture + Attribute Weight for Decision\\
    \textcolor{blue}{Correira~\textit{et al.}~\cite{correia2023face}} & 2023 & Face Verification & Rung 2 - M. P. & Attention + Explainability Masks Construction\\
    \textcolor{blue}{Bousnina~\textit{et al.}~\cite{bousnina2023rise}} & 2023 & Face Verification & Rung 2 - I. I. & RISE-Based Similarity/Dissimilarity Maps\\
    \textcolor{blue}{Knoche~\textit{et al.}~\cite{knoche2023explainable}} & 2023 & Face Verification & Rung 2 - I. I. + I. P. & Patch Replacement\\
    \textcolor{blue}{Lu and Ebrahimi~\cite{lu2023explanation}} & 2023 & Face Recognition & Rung 2 - I. I. & S-Rise\\
    \textcolor{blue}{Rajpal~\textit{et al.}~\cite{rajpal2023xai}} & 2023 & Face Recognition  & Rung 2 - I. I. & LIME Maps \\ % is lime only interpretable when we have interpertable features?????
    \textcolor{blue}{Neto~\textit{et al.}~\cite{neto2023pic}} & 2023 & Face Recognition & Rung 2 - I. P. & Interpretable Match Score \\
    \textcolor{blue}{Rodriguez~\textit{et al.}~\cite{rodriguez2023multi}} & 2023 & Quality Face Recognition & Rung 2 - T. R. P. & Enviromental Attributes \\
    \textcolor{orange}{Terhörst~\textit{et al.}~\cite{terhorst2021pixel}} & 2023 & Face quality for Face Recognition & Rung 2 - I. I. + I. P. & Pixel-level Quality Maps \\
    \textcolor{blue}{Fu~\textit{et al.}~\cite{fu2022towards}} & 2022 & Face Recognition Bias & Rung 1 & Differential Activation Maps \\
    \textcolor{orange}{Han~\textit{et al.}~\cite{han2022personalized}} & 2022 & Face Recognition & Rung 2 - T. R. P. & Personalized Kernels + Feature Maps \\

    \textcolor{blue}{Roy~\textit{et al.}~\cite{roy2022interpretable}} & 2022 & Heterogeneous Face Recognition & Rung 2 - M. P. + I. I. & Invariant Features\\
    \textcolor{blue}{Winter~\textit{et al.}~\cite{winter2022demystifying}} & 2022 & Face Recognition & Rung 2 - T. R. P. + I. P.  & Local Patch-based Features with Eexplainable Boosting Machine (EMB)\\
    \textcolor{orange}{Mery~\textit{et al.}~\cite{mery2022black}} & 2022 & Face Verification & Rung 1 & Saliency maps AVG contours \\
     \textcolor{orange}{Fu~\textit{et al.}~\cite{fu2022explainability}} & 2022 & Face quality for Face recogniton & Rung 1 & Score-CAM\cite{wang2020score} + Activation Maps\\
     \textcolor{blue}{Franco~\textit{et al.}~\cite{franco2022deep}} & 2022 & Face Recognition & Rung 2 - T. R. P. & Tikhonov regularizers \\

    \textcolor{orange}{Neto~\textit{et al.}~\cite{neto2021my,neto2021focusface}} & 2021 & Masked Face Recognition & Rung 2 - T. R. P.  + I.I. & Mask-Invariant Loss + Grad-CAM Visualisation\\
    \textcolor{blue}{Huber~\textit{et al.}~\cite{huber2021mask}} & 2021 & Masked Face Recognition & Rung 2 - T. R. P.  + I.I. & Mask-Invariant Knowledge Distillation\\

     \textcolor{blue}{Franco~\textit{et al.}~\cite{franco2021learn}} & 2021 & Face Recognition & Rung 2 - T. R. P. & Tikhonov regularizer\\
     \textcolor{orange}{Liu~\textit{et al.}~\cite{liu2021heterogeneous}} & 2021 & Heterogeneous Face Recognition & Rung 2 - T. R. P. + I. P. & Modality/Identity Disentangled Representation + Cross-modality Synthesis \\
     \textcolor{orange}{Anghelone~\textit{et al.}~\cite{anghelone2021explainable}} & 2021 & Face Recognition & Rung 1 & Heatmap-based Visualisation  \\
     \textcolor{orange}{Jiang and Zeng~\cite{jiang2021explainable}} & 2021 & Face Recognition & Rung 2 - T. R. P.  & Face Components Representation and Self-Attention based Reconstruction + Components Similarity Matrix \\
        \hline

    \textcolor{orange}{Williford~\textit{et al.}~\cite{williford2020explainable}} & 2020 & Face Recognition & Rung 2 - I.I. + T. R. P. + I. P. & DISE + subtree EBP +  Inpainting game \\
    \textcolor{orange}{Zee~\textit{et al.}~\cite{zee2019enhancing}} & 2019 & Face Recognition & Rung 1 & Guided Backpropagation \& CAM \\
    \textcolor{orange}{Yin~\textit{et al.}~\cite{yin2019towards}} & 2019 & Face Recognition &  Rung 2 - T. R. P. + I. I. & Spatial and Feature Activation Diversity Losses \\


    \hline
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Face Morphing}}} \\
    \hline
    \textcolor{blue}{Caldeira~\textit{et al.}~\cite{caldeira2023unveiling}} & 2023 & Face Morphing Detection & Rung 2 - M. P. + T. R. P. & Interpretable Score + Identity Disentanglement\\
    \textcolor{blue}{Dargaud~\textit{et al.}~\cite{dargaud2023principal}} & 2023 & Face Morphing Detection & Rung 1 & PCA-based Visualisation \\
    \textcolor{blue}{Dwivedi~\textit{et al.}~\cite{dwivedi2023efficient}} & 2023 & Face Morphing Detection & Rung 1 & Ensemble of Visualisations \\
    \textcolor{blue}{Neto~\textit{et al.}~\cite{Neto2022OrthMAD}} & 2022 & Face Morphing Detection & Rung 2 - T. R. P. & Orthogonal Identity Disentanglement\\
    \textcolor{blue}{Myhrvold~\textit{et al.}~\cite{myhrvold2022explainable}} & 2022 & Face Morphing Detection & Rung 1 & LRP \\
    \textcolor{orange}{Seibold~\textit{et al.}~\cite{seibold2021focused}}& 2021 & Face Morphing Attack Detection & Rung 1 & Focused LRP \\

    
    \multicolumn{5}{|c|}{\makecell{\textbf{Face PAD}}} \\
    \hline
    \textcolor{blue}{Prasad~\textit{et al.}~\cite{prasad2022self}} & 2023 & Face PAD & Rung 2 - T. R. P. & Intermediate Depth Estimation\\
    \textcolor{blue}{Pan~\textit{et al.}~\cite{pan2022attention}} & 2022 & Face PAD & Rung 2 - T. R. P. &  Grad-CAM + Textual Explanations\\
    \textcolor{orange}{Fang~\textit{et al.}~\cite{fang2022learnable}} & 2022 & Face PAD & Rung 2 - T. R. P. & Multi-Scale Frequency Decomposition + Hierarchical Attention + t-SNE \\
    
     \textcolor{blue}{Bian~\textit{et al.}~\cite{bian2022learning}} & 2022 & Face PAD & Rung 2 - T. R. P. & Auxiliary Learning with Interpretable Cues \\% not 100% sure about this one
     \textcolor{orange}{Wang~\textit{et al.}~\cite{wang2022disentangled}} & 2022 & Face PAD & Rung 2 - T. R. P. & Live Features Disentanglement + t-SNE\\
     \textcolor{orange}{Sequeira~\textit{et al.}~\cite{sequeira2021exploratory}} & 2021 & Face PAD & Rung 1 & Grad-CAM Visualisation\\
     \textcolor{orange}{Chen~\textit{et al.}~\cite{chen2021dual}} & 2021 & 3D Mask Face PAD & Rung 1 & Grad-CAM Visualisation and t-SNE \\
     \textcolor{orange}{Neto~\textit{et al.}~\cite{neto2021myope}} & 2021 & Face PAD & Rung 1 & Grad-CAM Visualisation \\
     \textcolor{orange}{Aghdaie~\textit{et al.}~\cite{aghdaie2021attention}} & 2021 & Face PAD & Rung 2 - T. R. P. & Attention + Attention Maps Visualization \\ 
     \textcolor{orange}{Yu~\textit{et al.}~\cite{yu2020searching}} & 2020 &  Face PAD & Rung 2 - M. P. + T. R. P. & Central Difference Convolution + Depth-Map Estimation \\
    \textcolor{orange}{Pinto~\textit{et al.}~\cite{pinto2020leveraging}} & 2020 & Face PAD & Rung 1 & Grad-CAM Visualisation \\
    \textcolor{orange}{Wang~\textit{et al.}~\cite{wang2020deep}} & 2020 &  Face PAD & Rung 2 - T. R. P. & Temporal Depth-Map Estimation + t-SNE \\
    \textcolor{orange}{Shao~\textit{et al.}~\cite{shao2020regularized}} & 2020 & Face PAD & Rung 2 - T. R. P. & Meta-learning with Depth Regularization + Attention Map Visualization \\
    \textcolor{orange}{Liu~\textit{et al.}~\cite{liu2020disentangling}} & 2020 & Face PAD & Rung 2 - T. R. P. & Spoof-traces disentanglement \\
    \textcolor{orange}{Yang~\textit{et al.}~\cite{yang2019face}} & 2019 & Face PAD & Rung 2 - T. R. P.  & Patch-based Attention + Grad-CAM + t-SNE \\
    \textcolor{orange}{Jourabloo~\textit{et al.}~\cite{jourabloo2018face}} & 2018 & Face PAD & Rung 2 - T. R. P. & Spoof Noise Modeling  + t-SNE~\cite{JMLR:v9:vandermaaten08a} \\
    \textcolor{orange}{Liu~\textit{et al.}~\cite{liu2018learning}} & 2018 & Face PAD & Rung 2 - T. R. P. & rPPG Signal Extraction \\


    \hline


    \multicolumn{5}{|c|}{\makecell{\textbf{Face DeepFakes}}} \\
    \hline
    \textcolor{blue}{Mathews~\textit{et al.}~\cite{mathews2023explainable}} & 2023 & Face DeepFake Detection & Rung 1 &  Grad-CAM Visualisations\\
    \textcolor{blue}{Silva~\textit{et al.}~\cite{silva2022deepfake}} & 2022 & Face DeepFake Detection & Rung 1 &  Attention Maps\\
    \textcolor{orange}{Mazaheri and Roy-Chowdhury~\cite{mazaheri2022detection}} & 2022 & Face Manipulation Detection & Rung 1 & CAM \\ % Is this deepFake detection?
    \textcolor{blue}{Korshunov~\textit{et al.}~\cite{korshunov2022custom}} & 2022 & Face DeepFake Detection & Rung 1 &  t-SNE \\ %  used a multi-task approach for improved generalization and "explainability"
    \textcolor{orange}{Xu~\textit{et al.}~\cite{xu2022supervised} }& 2022 & Face DeepFake Detection & Rung 1  & UMAP and Heatmap Visualisation \\
    
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Face Emotion/Expression Recognition}}} \\
    \hline
    \textcolor{blue}{Nam~\textit{et al.}~\cite{nam4208671facialcuenet}} & 2023 & Face Expression Recognition & Rung 2 - T. R. P. & Spatio-Temporal Attention Maps + Facial cues\\
    \textcolor{blue}{Rathod~\textit{et al.}~\cite{rathod2022kids}} & 2022 & Children Emotion Recognition & Rung 1 & Grad-CAM + Grad-CAM++ + SoftGrad\\
    \textcolor{blue}{Cesarelli~\textit{et al.}~\cite{cesarelli2022emotion}} & 2022 & Face Emotion Recognition & Rung 1 & Grad-CAM Visualisations\\
    \textcolor{blue}{Zhu~\textit{et al.}~\cite{zhu2022explainable}} & 2022 & Face Emotion Recognition & Rung 1 & LRP\\
    \textcolor{blue}{Araf~\textit{et al.}~\cite{araf2022real}} & 2022 & Face Emotion Recognition & Rung 1 & Grad-CAM Visualisations\\
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Fingerprint PAD/Recognition}}} \\
    \hline
    \textcolor{blue}{Rai~\textit{et al.}~\cite{rai2023expressnet}} & 2023 & Fingerprint PAD & Rung 1 &  Heatmap Visualisation\\
    \textcolor{blue}{Ramachandra and Li~\cite{ramachandra2023finger}} & 2023 & Fingerphoto Verification & Rung 2 - I. I. & Grad-CAM + Occlusion Sensitivity Maps + LIME + Gradient Attribution\\
    \textcolor{orange}{Chowdhury~\textit{et al.}~\cite{chowdhury2020can}} & 2020 & Fingerprint Recognition & Rung 1 & Grad-CAM Visualisation\\
    
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Iris Recognition}}} \\
    \hline
    \textcolor{blue}{Boyd~\textit{et al.}~\cite{boyd2023human}} & 2023 & Post-mortem Iris Recognition & Rung 2 - I. I. &  Visual Patch-matching\\
    \textcolor{orange}{Kuehlkamp~\textit{et al.}~\cite{kuehlkamp2022interpretable}} & 2022 & Post-mortem Iris Recognition & Rung 1 &  Segmentation Masks + CAM Visualisations\\
    \textcolor{orange}{Hu~\textit{et al.}~\cite{hu2020end}} & 2020 & Iris Recognition & Rung 1 & Grad-CAM Visualisation\\
    \textcolor{orange}{Trokielewicz~\textit{et al.}~\cite{trokielewicz2019perception}} & 2018 & Cadaver Iris Recognition& Rung 1  & Grad-CAM Visualisation\\
    

    \multicolumn{5}{|c|}{\makecell{\textbf{Iris PAD}}} \\
    \hline
    \textcolor{orange}{Sharma and Ross~\cite{sharma2021viability}} & 2021 & Iris PAD& Rung 1 & Grad-CAM Visualisation and t-SNE \\
    \textcolor{orange}{Fang~\textit{et al.}~\cite{fang2021iris}} & 2021 & Iris PAD & Rung 2 - T. R. P. & Patch-based Supervision + Attention +  Score-Weighted CAM~\cite{zhang2021group}\\
    \textcolor{orange}{Chen and Ross~\cite{chen2021}} & 2021 & Iris PAD & Rung 2 - T. R. P. & Channel and Position Attention +  Grad-CAM \\

    \textcolor{orange}{Sharma~\textit{et al.}~\cite{sharma2020d}} & 2020 & Iris PAD & Rung 1 & Grad-CAM Visualisation and t-SNE \\
    \textcolor{orange}{Trokielewicz~\textit{et al.}~\cite{trokielewicz2018presentation}} & 2018 & Cadaver Iris PAD & Rung 1 & Grad-CAM Visualisation and Guided Backpropagation  \\
    \hline
    \\

    \multicolumn{5}{|c|}{\makecell{\textbf{Others}}} \\
    \hline
    \textcolor{blue}{Diaz~\textit{et al.}~\cite{diaz4395568explainable}} & 2023 & Signature Verification & Rung 2 - M. P. + T. P. & Universal Background Model(UBM) + Explainable Features \\
    \textcolor{blue}{Aquino~\textit{et al.}~\cite{aquino2022explaining}} & 2022 & Accelerometer User Identification & Rung 1 & Grad-CAM\\
    \textcolor{blue}{Lim~\textit{et al.}~\cite{lim2022detecting}} & 2022 & Voice DeepFake Detection & Rung 1 & Deep Taylor + LRP\\
    \textcolor{orange}{Algermissen and H{\"o}rnlein~\cite{algermissen2021person}} & 2021 & Footstep Person Recognition & Rung 1 & Grad-CAM \\
    \textcolor{orange}{Alshazly~\textit{et al.}~\cite{alshazly2021towards}} & 2021 & Ear Recognition & Rung 1 & Guided Grad-CAM \\
    
    \textcolor{orange}{Chandaliya and Nain~\cite{chandaliya2021child}} & 2021 & Face Age Estimation & Rung 2 - T. R. P. & Attention \\ % Remove from the table? They don't even mention explainability
    \textcolor{orange}{Joshi~\textit{et al.}~\cite{Joshi2021}} & 2021 & Fingerprint ROI Segmentation & Rung 2 - T. R. P. + I. P. &Monte Carlo Dropout + Uncertainty Map \\
    %\textcolor{orange}{Kao~\textit{et al.}~\cite{Kao2020AnOS}} & 2020 & Signature Verification & Rung 1 & - \\
    \textcolor{orange}{Pinto and Cardoso~\cite{pinto2020xecg}} & 2020 & ECG Biometric Identification & Rung 1 & Gradient-SHAP + DeepLIFT + Saliency Maps\\
    \textcolor{orange}{Ahmed~\textit{et al.}~\cite{ahmed2020race}} & 2020 & Ethnicity Estimation & Rung 1 & Grad-CAM \\
    \textcolor{orange}{Genovese~\textit{et al.}~\cite{Genovese2019}} & 2019 & Face Aging & Rung 1 & Cross- GAN Filter Similarity Index \\
    %\hline
\bottomrule
    %\end{tabular}
\end{longtable}
\end{small}
\end{center}
\end{landscape}






==> table_methods_that_use_xai.tex <==
% THE IDEA OF THIS TABLE IS TO SHOW SOME METHODS THAT SAY THAT ARE USING EXPLAINABILITY AND UNDERSTAND HOW THEY”SEE”EXPLAINABILITY. TO SHOW THE DIVERGENCE OF IDEAS AND THE LACK OF STANDARDS
% \begin{landscape}
% \begin{longtable}[h!]
%     \centering
%     \caption{Methods that leverage explainability methods to inspect the predictions of biometric systems. Some of these methods, promote interpretability through the usage of certain techniques, whereas others focus mostly on explaining the predictions. }
%     \label{tab:xai4bio_works}
%     \begin{tabular}{lclll}
%     \toprule
%         \textbf{Method} & \textbf{Year} & \textbf{Modality} & \textbf{Promote Interpretability} & \textbf{xAI Method} \\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Face Recognition}}} \\
%     \midrule
%     Yin~\textit{et al.}~\cite{yin2019towards} & 2019 & Face Recognition &  Feature and Spatial Activation Diversity loss & Locations of Filter Response \\
%     Zee~\textit{et al.}~\cite{zee2019enhancing} & 2019 & Face Recognition & Siamese training & Guided Backpropagation \& CAM \\
%     Williford~\textit{et al.}~\cite{williford2020explainable} & 2020 & Face Recognition & DISE, subtree EBP & Inpainting game \\
%     Neto~\textit{et al.}~\cite{neto2021my,neto2021focusface} & 2021 & Masked Face Recognition & Strong Constraints & Grad-CAM\\
%     Jiang and Zeng~\cite{jiang2021explainable} & 2021 & Face Recognition &  Local Feature Refine and Self-Attention based Reconstruction modules & Similarity Matrix \\
%     Liu~\textit{et al.}~\cite{liu2021heterogeneous} & 2021 & Heterogeneous Face Recognition & Symmetric adversarial loss & HFIDR \\
%     \textcolor{orange}{Anghelone~\textit{et al.}~\cite{anghelone2021explainable}} & 2021 & Face Recognition &  & \\
%     Mery~\textit{et al.}~\cite{mery2022black} & 2022 & Face Verification & - & Saliency maps AVG contours \\
%     \textcolor{red}{Fu~\textit{et al.}~\cite{fu2022explainability}} & 2022 & \textcolor{red}{Face quality for Face recogniton} & & \\
%     Han~\textit{et al.}~\cite{han2022personalized} & 2022 & Face Recognition & Personalized Kernels & Feature Maps \\
    

%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Face PAD}}} \\
%     \midrule
%     Liu~\textit{et al.}~\cite{liu2018learning} & 2018 & Face PAD & Aux. Supervision & - \\
%     Jourabloo~\textit{et al.}~\cite{jourabloo2018face} & 2018 & Face PAD & Spoof Pattern Estimation & t-SNE \\
%     Yang~\textit{et al.}~\cite{yang2019face} & 2019 & Face PAD & Aux. Supervision & t-SNE \\
%     Pinto~\textit{et al.}~\cite{pinto2020leveraging} & 2020 & Face PAD & - & Grad-CAM \\
%     Liu~\textit{et al.}~\cite{liu2020disentangling} & 2020 & Face PAD & Aux. Supervision & - \\
%     Shao~\textit{et al.}~\cite{shao2020regularized} & 2020 & Face PAD & Depth-Map Estimation & Attention Maps Visualization \\
%     Wang~\textit{et al.}~\cite{wang2020deep} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE~\cite{JMLR:v9:vandermaaten08a} \\
%     Yu~\textit{et al.}~\cite{yu2020searching} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE \\
%     Sequeira~\textit{et al.}~\cite{sequeira2021exploratory} & 2021 & Face PAD & - & Grad-CAM \\
%     Aghdaie~\textit{et al.}~\cite{aghdaie2021attention} & 2021 & Face PAD & Attention & Attention Maps Visualization \\
%     Chen~\textit{et al.}~\cite{chen2021dual} & 2021 & 3D Mask Face PAD & - & Grad-CAM and t-SNE \\
%     Neto~\textit{et al.}~\cite{neto2021myope} & 2021 & Face PAD & - & Grad-CAM \\
%     \textcolor{orange}{Fang~\textit{et al.}~\cite{fang2022learnable}} & 2022 & Face PAD & Attention & t-SNE \\
%     \textcolor{red}{Wang~\textit{et al.}~\cite{wang2022disentangled}} & 2022 & Face PAD & Spoof Maps & t-SNE\\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Iris PAD}}} \\
%     \midrule
%     Trokielewicz~\textit{et al.}~\cite{trokielewicz2018presentation} & 2018 & Cadaver Iris PAD & - & Grad-CAM and Guided backpropagation  \\
%     Sharma~\textit{et al.}~\cite{sharma2020d} & 2020 & Iris PAD & - & t-SNE and Grad-CAM \\
%     Fang~\textit{et al.}~\cite{fang2021iris} & 2021 & Iris PAD & Aux. Supervision, Attention &  Score-Weighted CAM~\cite{zhang2021group}\\
%     Chen~\textit{et al.}~\cite{chen2021} & 2021 & Iris PAD & Attention & Grad-CAM \\
%     \textcolor{purple}{Sharma and Ros}s~\cite{sharma2021viability} & 2021 & Iris PAD& - & Grad-CAM and t-SNE \\
%     \midrule
%     \multicolumn{5}{c}{\makecell{\textbf{Others}}} \\
%     \midrule
%     \textcolor{purple}{Genovese}~\textit{et al.}~\cite{Genovese2019} & 2019 & Face Aging & - & CGFSI \\
%     Trokielewicz~\textit{et al.}~\cite{trokielewicz2019perception} & 2018 & Cadaver Iris Recognition& -  & Grad-CAM \\
%     Hu~\textit{et al.}~\cite{hu2020end} & 2020 & Iris Recognition & - & Grad-CAM \\
%     Kao~\textit{et al.}~\cite{Kao2020AnOS} & 2020 & Signature Verification & - & - \\
%     Pinto~\textit{et al.}~\cite{pinto2020xecg} & 2020 & ECG Biometric Identification & - & Miscellaneous\\
%     Ahmed~\textit{et al.}~\cite{ahmed2020race} & 2020 & Race Estimation & - & Grad-CAM \\
%     Chowdhury~\textit{et al.}~\cite{chowdhury2020can} & 2020 & Fingerprint Recognition & - & Grad-CAM \\
%     Chandaliya and Nain~\cite{chandaliya2021child} & 2021 & Face Age Estimation & Attention & - \\
%     Joshi~\textit{et al.}~\cite{Joshi2021} & 2021 & Fingerprint ROI Segmentation & Monte Carlo Dropout & Uncertainty Map \\
%     \textcolor{purple}{Seibold}~\textit{et al.}~\cite{seibold2021focused}& 2021 & Face Morphing Attack Detection & Focused LRP & Focused LRP \\
%     Ortega~\textit{et al.}~\cite{ortega2021symbolic} & 2021 & Automatic Recruitment & LFIT~\cite{Ribeiro2016StudiesOL} & Declarative Explanation \\
%     Algermissen and H{\"o}rnlein~\cite{algermissen2021person} & 2021 & Footstep Person Recognition & - & Grad-CAM \\
%     Alshazly~\textit{et al.}~\cite{alshazly2021towards} & 2021 & Ear Recognition & - & Guided Grad-CAM \\
%     \textcolor{orange}{Mazaheri~\textit{et al.}~\cite{mazaheri2022detection}} & 2022 & Face Manipulation Detection & - & Grad-CAM \\
%     \textcolor{purple}{Kuehlkamp~\textit{et al.}~\cite{kuehlkamp2022interpretable}} & 2022 & Cadaver Iris Recognition & - & Segmentation Masks and CAM \\
%     \textcolor{orange}{Gelberg~\textit{et al.}~\cite{gelberg2022skeleton}} & 2022 & Typing style Recognition & Joint-based recognition & t-SNE \\
%     \textcolor{purple}{Xu~\textit{et al.}~\cite{xu2022supervised}} & 2022 & DeepFake Detection & -  & UMAP and Heatmaps \\
         

         
         
         


%     \bottomrule
%     \end{tabular}
    
% \end{longtable}
% \end{landscape}

\begin{landscape}
\begin{center}\begin{small}
\begin{longtable}{|p{0.22\textheight}p{0.02\textheight}p{0.25\textheight}p{0.29\textheight}p{0.270\textheight}|}

    \caption{Methods that leverage explainability methods to inspect the predictions of biometric systems. Some of these methods, promote interpretability through the usage of certain techniques, whereas others focus mostly on explaining the predictions.}\label{tab:xai4bio_works}\\
    \toprule
    \textbf{Method} & \textbf{Year} & \textbf{Modality} & \textbf{Promote Interpretability} & \textbf{xAI Method} \\
    \hline
    \endhead

    %\endfoot
    
    \multicolumn{5}{|c|}{\makecell{\textbf{Face Recognition}}} \\
    \hline
    \textbf{Yin}~\textit{et al.}~\cite{yin2019towards} & 2019 & Face Recognition &  FAD and SAD losses & Locations of Filter Response \\
    \textbf{Zee}~\textit{et al.}~\cite{zee2019enhancing} & 2019 & Face Recognition & Siamese training & Guided Backpropagation \& CAM \\
    \textbf{Williford}~\textit{et al.}~\cite{williford2020explainable} & 2020 & Face Recognition & DISE, subtree EBP & Inpainting game \\
    \textbf{Neto}~\textit{et al.}~\cite{neto2021my,neto2021focusface} & 2021 & Masked Face Recognition & Strong Loss Constraints & Grad-CAM\\
    \textbf{Jiang and Zeng}~\cite{jiang2021explainable} & 2021 & Face Recognition &  Local Feature Refine and Self-Attention based Reconstruction modules & Similarity Matrix \\
    \textbf{Liu}~\textit{et al.}~\cite{liu2021heterogeneous} & 2021 & Heterogeneous Face Recognition & Symmetric adversarial loss & HFIDR \\
    \textbf{Anghelone}~\textit{et al.}~\cite{anghelone2021explainable} & 2021 & Face Recognition & - & Heatmap-based visualization  \\
    \textbf{Terhörst}~\textit{et al.}~\cite{terhorst2021pixel} & 2021 & Face quality for Face Recognition & Pixel quality estimation & Pixel quality-based heatmap \\
    \textbf{Mery}~\textit{et al.}~\cite{mery2022black} & 2022 & Face Verification & - & Saliency maps AVG contours \\
    \textbf{Fu}~\textit{et al.}~\cite{fu2022explainability} & 2022 & Face quality for Face recogniton & - & Score-CAM\cite{wang2020score} \& Activation Maps\\%Statistics of Activation Maps\\
    \textbf{Han}~\textit{et al.}~\cite{han2022personalized} & 2022 & Face Recognition & Personalized Kernels & Feature Maps \\
    \hline
    \multicolumn{5}{|c|}{\makecell{\textbf{Face PAD}}} \\
    \hline
    \textbf{Liu}~\textit{et al.}~\cite{liu2018learning} & 2018 & Face PAD & Aux. Supervision & - \\
    \textbf{Jourabloo}~\textit{et al.}~\cite{jourabloo2018face} & 2018 & Face PAD & Spoof Pattern Estimation & t-SNE~\cite{JMLR:v9:vandermaaten08a} \\
    \textbf{Yang}~\textit{et al.}~\cite{yang2019face} & 2019 & Face PAD & Aux. Supervision & t-SNE \\
    \textbf{Pinto}~\textit{et al.}~\cite{pinto2020leveraging} & 2020 & Face PAD & - & Grad-CAM \\
    \textbf{Liu}~\textit{et al.}~\cite{liu2020disentangling} & 2020 & Face PAD & Aux. Supervision & - \\
    \textbf{Shao}~\textit{et al.}~\cite{shao2020regularized} & 2020 & Face PAD & Depth-Map Estimation & Attention Maps Visualization \\
    \textbf{Wang}~\textit{et al.}~\cite{wang2020deep} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE \\
    \textbf{Yu}~\textit{et al.}~\cite{yu2020searching} & 2020 &  Face PAD & Depth-Map Estimation & t-SNE \\
    \textbf{Sequeira}~\textit{et al.}~\cite{sequeira2021exploratory} & 2021 & Face PAD & - & Grad-CAM \\
    \textbf{Aghdaie}~\textit{et al.}~\cite{aghdaie2021attention} & 2021 & Face PAD & Attention & Attention Maps Visualization \\
    \textbf{Chen}~\textit{et al.}~\cite{chen2021dual} & 2021 & 3D Mask Face PAD & - & Grad-CAM and t-SNE \\
    \textbf{Neto}~\textit{et al.}~\cite{neto2021myope} & 2021 & Face PAD & - & Grad-CAM \\
    \textbf{Fang}~\textit{et al.}~\cite{fang2022learnable} & 2022 & Face PAD & Attention & t-SNE \\
    \textbf{Wang}~\textit{et al.}~\cite{wang2022disentangled} & 2022 & Face PAD & Spoof Maps & t-SNE\\
    %\hline
\bottomrule
    %\end{tabular}
\end{longtable}
\end{small}
\end{center}
\end{landscape}

\begin{landscape}
\begin{center}\begin{small}
\begin{longtable}{|p{0.22\textheight}p{0.02\textheight}p{0.25\textheight}p{0.29\textheight}p{0.25\textheight}|}

    \caption{Continuation of the methods that leverage explainability methods to inspect the predictions of biometric systems. Some of these methods, promote interpretability through the usage of certain techniques, whereas others focus mostly on explaining the predictions.}\label{tab:xai4bio_works2}\\
    \toprule
    \textbf{Method} & \textbf{Year} & \textbf{Modality} & \textbf{Promote Interpretability} & \textbf{xAI Method} \\
    \hline
    \endhead
    \multicolumn{5}{|c|}{\makecell{\textbf{Iris PAD}}} \\
    \hline
    \textbf{Trokielewicz}~\textit{et al.}~\cite{trokielewicz2018presentation} & 2018 & Cadaver Iris PAD & - & Grad-CAM and Guided backpropagation  \\
    \textbf{Sharma}~\textit{et al.}~\cite{sharma2020d} & 2020 & Iris PAD & - & t-SNE and Grad-CAM \\
    \textbf{Fang}~\textit{et al.}~\cite{fang2021iris} & 2021 & Iris PAD & Aux. Supervision, Attention &  Score-Weighted CAM~\cite{zhang2021group}\\
    \textbf{Chen}~\textit{et al.}~\cite{chen2021} & 2021 & Iris PAD & Attention & Grad-CAM \\
    \textbf{Sharma and Ross}~\cite{sharma2021viability} & 2021 & Iris PAD& - & Grad-CAM and t-SNE \\
    \hline
    \multicolumn{5}{|c|}{\makecell{\textbf{Others}}} \\
    \hline
    \textbf{Genovese}~\textit{et al.}~\cite{Genovese2019} & 2019 & Face Aging & - & CGFSI \\
    \textbf{Trokielewicz}~\textit{et al.}~\cite{trokielewicz2019perception} & 2018 & Cadaver Iris Recognition& -  & Grad-CAM \\
    \textbf{Hu}~\textit{et al.}~\cite{hu2020end} & 2020 & Iris Recognition & - & Grad-CAM \\
    \textbf{Kao}~\textit{et al.}~\cite{Kao2020AnOS} & 2020 & Signature Verification & - & - \\
    \textbf{Pinto}~\textit{et al.}~\cite{pinto2020xecg} & 2020 & ECG Biometric Identification & - & Miscellaneous\\
    \textbf{Ahmed}~\textit{et al.}~\cite{ahmed2020race} & 2020 & Race Estimation & - & Grad-CAM \\
    \textbf{Chowdhury}~\textit{et al.}~\cite{chowdhury2020can} & 2020 & Fingerprint Recognition & - & Grad-CAM \\
    \textbf{Chandaliya and Nain}~\cite{chandaliya2021child} & 2021 & Face Age Estimation & Attention & - \\
    \textbf{Joshi}~\textit{et al.}~\cite{Joshi2021} & 2021 & Fingerprint ROI Segmentation & Monte Carlo Dropout & Uncertainty Map \\
    \textbf{Seibold}~\textit{et al.}~\cite{seibold2021focused}& 2021 & Face Morphing Attack Detection & - & Focused LRP \\
    Ortega~\textit{et al.}~\cite{ortega2021symbolic} & 2021 & Automatic Recruitment & Learning from Interpretation Transition(LFIT)~\cite{Ribeiro2016StudiesOL} & Declarative Explanation \\
    \textbf{Algermissen} and H{\"o}rnlein~\cite{algermissen2021person} & 2021 & Footstep Person Recognition & - & Grad-CAM \\
    \textbf{Alshazly}~\textit{et al.}~\cite{alshazly2021towards} & 2021 & Ear Recognition & - & Guided Grad-CAM \\
    \textbf{Mazaheri}~\textit{et al.}~\cite{mazaheri2022detection} & 2022 & Face Manipulation Detection & - & CAM \\
    \textbf{Kuehlkamp}~\textit{et al.}~\cite{kuehlkamp2022interpretable} & 2022 & Cadaver Iris Recognition & - & Segmentation Masks and CAM \\
    Gelberg~\textit{et al.}~\cite{gelberg2022skeleton} & 2022 & Typing style Recognition & Joint-based recognition & t-SNE \\
    \textbf{Xu}~\textit{et al.}~\cite{xu2022supervised} & 2022 & DeepFake Detection & -  & UMAP and Heatmaps \\
        
    \bottomrule


    
    %\end{tabular}
\end{longtable}
\end{small}
\end{center}
\end{landscape}




